Follow-up Analyses to the O3 LIGO-Virgo-KAGRA Lensing Searches

Along their path from source to observer, gravitational waves may be gravitationally lensed by massive objects. This results in distortions of the observed signal which can be used to extract new information about fundamental physics, astrophysics, and cosmology. Searches for these distortions amongst the observed signals from the current detector network have already been carried out, though there have as yet been no confident detections. However, predictions of the observation rate of lensing suggest detection in the future is a realistic possibility. Therefore, preparations need to be made to thoroughly investigate the candidate lensed signals. In this work, we present some of the follow-up analyses and strategies that could be applied to assess the significance of such events and ascertain what information may be extracted about the lens-source system from such candidate signals by applying them to a number of O3 candidate events, even if these signals did not yield a high significance for any of the lensing hypotheses. For strongly-lensed candidates, we verify their significance using a background of simulated unlensed events and statistics computed from lensing catalogs. We also look for potential electromagnetic counterparts. In addition, we analyse in detail a candidate for a strongly-lensed sub-threshold counterpart that is identified by a new method. For microlensing candidates, we perform model selection using a number of lens models to investigate our ability to determine the mass density profile of the lens and constrain the lens parameters. We also look for millilensing signatures in one of the lensed candidates. Applying these additional analyses does not lead to any additional evidence for lensing in the candidates that have been examined. However, it does provide important insight into potential avenues to deal with high-significance candidates in future observations.

==> authors.tex <==
\collaboration{\textbf{Editorial Team}}

\author[Janquart et al.]{
\textit{\textbf{Editorial Team}} \\

\author{J.Janquart$^{*}$}
\affiliation{\grasp}
\affiliation{\nikhef}
\email{$^{*}$j.janquart@uu.nl}

\author{M. Wright$^{\dagger}$}
\affiliation{\glasgow}
\email{$^{\dagger}$m.wright.3@research.gla.ac.uk}

\author{S. Goyal}
\affiliation{\tata}

%\collaboration{\textbf{Analysts}}
\textit{\textbf{Analysts}}

\author{J. C. L. Chan}
\affiliation{\niels}

\author{A. Ganguly}
\affiliation{\iucaa}
\affiliation{\tata}

\author{\'A. Garr\'on}
\affiliation{\balearic}

\author{D. Keitel}
\affiliation{\balearic}
\affiliation{\portsmouth}

\author{A. K. Y. Li}
\affiliation{\ligocit}

\author{A. Liu}
\affiliation{\chuk}

\author{R. K. L. Lo}
\affiliation{\ligocit}

\author{A. Mishra}
\affiliation{\iucaa}

\author{A. More}
\affiliation{\iucaa}
\affiliation{\kavliJ}

\author{H. Phurailatpam}
\affiliation{\chuk}

\author{P. Prasia}
\affiliation{\iucaa}


%\collaboration{\textbf{Contributors}}
\textit{\textbf{Contributors}}


\author{P. Ajith}
\affiliation{\tata}
\affiliation{\cifar}

\author{S. Biscoveanu}
\affiliation{\ligomit}
\affiliation{\kavli}

\author{P. Cremonese}
\affiliation{\balearic}

\author{J.R. Cudell}
\affiliation{\liege}

\author{J. M. Ezquiaga}
\affiliation{\niels}

\author{J. Garcia-Bellido}
\affiliation{\madrid}

\author{O. A. Hannuksela}
\affiliation{\chuk}

\author{K. Haris}
\affiliation{\nikhef}
\affiliation{\grasp}

\author{I. Harry}
\affiliation{\portsmouth}

\author{M. Hendry}
\affiliation{\glasgow}

\author{S. Husa}
\affiliation{\balearic}

\author{S. Kapadia}
\affiliation{\iucaa}

\author{T. G. F. Li}
\affiliation{\kul}
\affiliation{\kuleng}
\affiliation{\chuk}

\author{I. Maga\~na Hernandez}
\affiliation{\milwaukee}
\affiliation{\CMU}

\author{S. Mukherjee}
\affiliation{\tatamumbai}

\author{E. Seo}
\affiliation{\glasgow}

\author{C. Van Den Broeck}
\affiliation{\grasp}
\affiliation{\nikhef}

\author{J. Veitch}
\affiliation{\glasgow}
}

==> macros/overall_macros.tex <==
\newtoggle{cleancomments}
\togglefalse{cleancomments}

\newcommand{\NUMEVENTS}{39}

\newcommand{\IMRD}{\textsc{IMRPhenomD}\xspace}
\newcommand{\IMRP}{\textsc{IMRPhenomPv2}\xspace}
\newcommand{\IMRPHM}{\textsc{IMRPhenomPv3HM}\xspace}
\newcommand{\IMRPNRT}{\textsc{IMRPhenomPv2\_NRTidal}\xspace}
\newcommand{\IMRXPHM}{\textsc{IMRPhenomXPHM}\xspace}
\newcommand{\NRSur}{\textsc{NRSur7dq4}\xspace}

\newcommand{\cmark}{\ding{51}}
\newcommand{\xmark}{\ding{55}}

\newcommand{\linf}{\textsc{LALInference}\xspace}
\newcommand{\linfmcmc}{\textsc{LALInferenceMCMC}\xspace}
\newcommand{\linfnest}{\textsc{LALInferenceNest}\xspace}
\newcommand{\lal}{\textsc{LALSuite}\xspace}
\newcommand{\gstlal}{\textsc{GstLAL}\xspace}
\newcommand{\pycbc}{\textsc{PyCBC}\xspace}
\newcommand{\cwb}{\textsc{cWB}\xspace}
\newcommand{\hanabi}{\textsc{hanabi}\xspace}
\newcommand{\bilby}{\textsc{Bilby}\xspace}
\newcommand{\bayestar}{\textsc{Bayestar}\xspace}

\newcommand{\gw}[1][]{gravitational wave#1 (GW#1)\renewcommand{\gw}[1][]{GW##1\xspace}\xspace}
\newcommand{\cbc}[1][]{compact binary coalescence#1 (CBC#1)\renewcommand{\cbc}[1][]{CBC##1\xspace}\xspace}
\newcommand{\bns}[1][]{binary neutron star#1 (BNS#1)\renewcommand{\bns}[1][]{BNS##1\xspace}\xspace}
\newcommand{\bbh}[1][]{binary black hole#1 (BBH#1)\renewcommand{\bbh}[1][]{BBH##1\xspace}\xspace}
\newcommand{\nsbh}[1][]{neutron star--black hole#1 (NSBH#1)\renewcommand{\nsbh}[1][]{NSBH##1\xspace}\xspace}
\newcommand{\pe}{parameter estimation (PE)\renewcommand{\pe}{PE\xspace}\xspace}
\newcommand{\pisn}{pair instability supernova (PISN)\renewcommand{\pisn}{PISN\xspace}\xspace}
\newcommand{\kde}[1][]{kernel density estimator#1 (KDE#1)\renewcommand{\kde}[1][]{KDE##1\xspace}\xspace}
\newcommand{\fap}[1][]{false-alarm probability#1 (FAP#1)\renewcommand{\fap}[1][]{FAP##1\xspace}\xspace}
\newcommand{\far}[1][]{false-alarm rate#1 (FAR#1)\renewcommand{\far}[1][]{FAR##1\xspace}\xspace}
\newcommand{\sgwb}{stochastic GW background (SGWB)\renewcommand{\sgwb}{SGWB\xspace}\xspace}
\newcommand{\snr}[1][]{signal-to-noise ratio#1 (SNR#1)\renewcommand{\snr}[1][]{SNR##1\xspace}\xspace}

\newcommand{\Msun}{\ensuremath{\text{M}_\odot}}
\newcommand{\Mc}{\ensuremath{\mathcal{M}}}

\newcommand{\posstatistic}{\mathcal{B}^{\rm overlap}}
\newcommand{\lensedhyp}{\mathcal{H}_{\rm SL}}
\newcommand{\notlensedhyp}{\mathcal{H}_{\rm U}}
\newcommand{\cohratio}{\mathcal{C}^\mathrm{L}_\mathrm{U}}
\newcommand{\Blu}{\mathcal{B}^\mathrm{L}_\mathrm{U}}

\newcommand{\BMLU}{\mathcal{B}_\mathrm{U}^\mathrm{ML}}
\newcommand{\zL}{z_\mathrm{l}}
\newcommand{\MzL}{M^z_\mathrm{L}}

\def\Rlu{{\mc{R}_\textsc{u}^\ell}}
\def\fdm{{f_\mathrm{DM}}}
\def\LambdaL{{\Lambda_\ell}}


==> macros/statistics_macros.tex <==
\newcommand{\RateAboveTwo}{\ensuremath{3.3_{-0.7}^{+0.9}\times{10^{-4}}}}
\newcommand{\RateAboveThirty}{\ensuremath{2.7_{-0.1}^{+0.2}\times{10^{-5}}}}

\newcommand{\RateModelAGalaxyDouble}{\ensuremath{0.8\text{--}4.3\times{10^{-4}}}}
\newcommand{\RateModelAGalaxySingle}{\ensuremath{2.6\text{--}8.6\times{10^{-4}}}}
\newcommand{\RateModelAClusterDouble}{\ensuremath{0.4\text{--}1.7\times{10^{-4}}}}
\newcommand{\RateModelAClusterSingle}{\ensuremath{1.3\text{--}3.7\times{10^{-4}}}}

\newcommand{\RateModelBGalaxyDouble}{\ensuremath{0.5\text{--}14.0\times{10^{-4}}}}
\newcommand{\RateModelBGalaxySingle}{\ensuremath{1.2\text{--}24.0\times{10^{-4}}}}
\newcommand{\RateModelBClusterDouble}{\ensuremath{0.4\text{--}7.0\times{10^{-4}}}}
\newcommand{\RateModelBClusterSingle}{\ensuremath{0.8\text{--}11.0\times{10^{-4}}}}

